Towards Optimisation of Collaborative Question Answering over Knowledge Graphs

Collaborative Question Answering (CQA) frameworks for knowledge graphs aim at integrating existing question answering (QA) components for implementing sequences of QA tasks (i.e. QA pipelines). The research community has paid substantial attention to CQAs since they support reusability and scalability of the available components in addition to the flexibility of pipelines. CQA frameworks attempt to build such pipelines automatically by solving two optimisation problems: 1) local collective performance of QA components per QA task and 2) global performance of QA pipelines. In spite offering several advantages over monolithic QA systems, the effectiveness and efficiency of CQA frameworks in answering questions is limited. In this paper, we tackle the problem of local optimisation of CQA frameworks and propose a three fold approach, which applies feature selection techniques with supervised machine learning approaches in order to identify the best performing components efficiently. We have empirically evaluated our approach over existing benchmarks and compared to existing automatic CQA frameworks. The observed results provide evidence that our approach answers a higher number of questions than the state of the art while reducing: i) the number of used features by 50% and ii) the number of components used by 76%.

==> storyline.tex <==
In this paper, we evaluate three things:
1) what is the component wise performance 
based on different type of features in question, as till now QA systems and components were reporting overall accurecy,
so its hard to comment on pitfalls of the QA community, and the components. We are more interested in understanding the pitfalls and way forward to improve the QA components, also do open new research directions.

2) In Last year VLDBs paper, \url{http://www.vldb.org/pvldb/vol10/p565-cui.pdf} they have proposed a concept of hybrid QA systems. Means they combined their QA system with other QA system, and improved the accuracy. For details see page 574 Table 11 in the paper. We did similar thing in WWW paper by combining QA components. So in our paper, we combine different components to show that not always this hypothesis is generalisable. 

3) then we test the relatedness in the components by doing some data analytic to understand which components shows similar behaviours across features. 

Some VLDB evaluation paper: http://www.vldb.org/pvldb/vol10/p1010-liu.pdf
                            http://www.vldb.org/pvldb/vol10/p553-harding.pdf
                            http://www.vldb.org/pvldb/vol8/p281-lu.pdf
